Exploring Effects of Random Walk Based Minibatch Selection Policy on Knowledge Graph Completion

In this paper, we have explored the effects of different minibatch sampling techniques in Knowledge Graph Completion. Knowledge Graph Completion (KGC) or Link Prediction is the task of predicting missing facts in a knowledge graph. KGC models are usually trained using margin, soft-margin or cross-entropy loss function that promotes assigning a higher score or probability for true fact triplets. Minibatch gradient descent is used to optimize these loss functions for training the KGC models. But, as each minibatch consists of only a few randomly sampled triplets from a large knowledge graph, any entity that occurs in a minibatch, occurs only once in most cases. Because of this, these loss functions ignore all other neighbors of any entity, whose embedding is being updated at some minibatch step. In this paper, we propose a new random-walk based minibatch sampling technique for training KGC models that optimizes the loss incurred by a minibatch of closely connected subgraph of triplets instead of randomly selected ones. We have shown results of experiments for different models and datasets with our sampling technique and found that the proposed sampling algorithm has varying effects on these datasets/models. Specifically, we find that our proposed method achieves state-of-the-art performance on the DB100K dataset.

==> mycontent/donot_submit.tex <==
\appendix
\section{Minibatch Properties}
\label{subsec:mini-vs-nl}
To motivate the new loss function, we will first look at a few properties of the minibatch used for training these models. In Figure \ref{fig:wn18rr-mini-stats} and \ref{fig:fb15k237-mini-stats}, we have shown degree distribution of the actual graph and randomly sampled minibatches used for training. To get a less erroneous estimate of degree distribution for the minibatches, we consider the average of degree distribution for all minibatches across a complete epoch. From these figures it is clear that, no matter the batch size, these minibatches are always a very sparse selection of triplets from the complete graph. 

In comparison to this, if we augment the minibatches with neighboring triplets, it decreases the sparsity of the minibatches by a lot. For the examples given in Figure \ref{fig:fb15k237-nl-stats} and \ref{fig:wn18rr-nl-stats}, we can observe nearly a 60\% drop in number of entities in minibatch with degree 1.

\subsection{Random Walk with Fly-Back}
Random walk is a graph sampling method where one takes a step by randomly choosing from all different options. In the simplest for of random walk, one moves to a neighboring vertex of the current one randomly selected from all of its neighbors.

\subsection{The Generalized Neighbors' Loss}

As we saw in the previous section, in most cases these randomly minibatches will contain any entity only once, as subject or object entity in some triplet. This causes the training algorithm to ignore how these updates affect the neighbors of the entities present in the current minibatch. Based on this notion and the observations from Section \ref{subsec:mini-vs-nl}, we modify the generalized loss function presented in Equation \ref{eqn:vanilla-loss} to also consider the neighboring triplets around the entities in a randomly selected minibatch. The new loss function is given by,

\begin{align}
    L(T_m) = \sum_{t \in T_m} \frac{1}{(1+|T^N_t|)} \Bigg( \sum_{t'\in T'_t} l_\Theta(\phi(t), \phi(t')) \nonumber \\
    + \sum_{n\in T^N_t} \sum_{n'\in T'_n} l_\Theta(\phi(n), \phi(n')) \Bigg) \label{eqn:NLoss}
\end{align}

where, $T_t^N$ is the set of triplets whose either subject or object entity coincides with subject or object entity of $t=(s,r,o)$.
% $T_m^G$ is union of $T_m$ and the set of triplets in $T$ for which either of the entities lies within $T_m$.
\begin{align}
    T_t^N = & \{(s',r',o') \in T | t=(s,r,o), s=s' \lor o=o'\} \setminus \{t\} \label{eqn:neighbors}
\end{align}

\section{Gradient Analysis}

\paragraph{SHOW THAT}
\begin{itemize}
 \item \textit{Using random walk to select minibatch guarantees to increase the number of times an entity vector (trainable parameter) appears in the loss function.}
 \item \textit{RWR increases average degree of minibatch subgraph}
 \item \textit{Above two facts lead to a more stable estimate for the gradient w.r.t to any involved entity vector.}
\end{itemize}


To understand the reason for improvement in the models with Neighbors' Loss, we need to look into the gradient of per-minibatch loss function with respect to any entity embedding being updated. First lets look at the gradient of the generalized vanilla-loss with respect to entity embedding of s, for a minibatch $T_m$.

\begin{align}
\nabla_{e_s} L(T_m) = \sum_{t \in T_{ms}} \nabla_{e_s} l(\phi(t), \phi(t')) \nonumber
\end{align}
where, $T_{ms}$ is the set of triplets in $T_m$ that contains entity s as either subject or object. $e_s$ is the embedding of the entity s.

Following is the gradient of the Neighbors' loss for minibatch $T_m$, with respect to the embedding of same entity s.

\begin{align}
\nabla_{e_s} L(T_m) = \sum_{t \in T_{ms}} \frac{1}{(1+|T^N_t|)} \Big( \sum_{t \in T'} \nabla_{e_s} l_\Theta(\phi(t), \phi(t')) \nonumber \\ + \sum_{n\in T^N_t} \sum_{n'\in T'_n} \nabla_{e_s} l_\Theta(\phi(n), \phi(n')) \Big) \label{eqn:grad-nloss}
\end{align}

As we can see in Equation \ref{eqn:grad-nloss}, there are more number of triplets in the loss function contributing towards the gradient in NLoss. Because of this, with NLoss, the gradient in every minibatch will have less variance compared to vanilla-loss. This is also shown through empirical results in \ref{fig:gradients} and is explained further in section \ref{sec:experiments}.


\section{Implementing the Neighbors' Loss}
We have used OpenKE \cite{han2018openke} and RotatE \cite{rotate} implementations of various KGC models to experiment with the proposed minibatch selection algorithm.
We implement Neighbors' Loss for all the models described in Section \ref{sec:background}. Although a generalized loss function (equation \ref{eqn:NLoss}) exists for Neighbors' Loss, the actual implementation of it for each model differs due to the type of loss functions which were originally used in the implementation of the models. For each of these models, we have taken their open-sourced implementations from Github \cite{han2018openke} \footnote{OpenKE: \url{https://github.com/thunlp/OpenKE/tree/OpenKE-PyTorch} \\RotatE: \url{https://github.com/DeepGraphLearning/KnowledgeGraphEmbedding} \\TuckER: \url{https://github.com/ibalazevic/TuckER}}. We augmented the random minibatch selection method for the models with neighboring triplets as per the requirements of the proposed loss function. Also to prevent the minibatches from growing too large in size, we put a cap on maximum number neighbors that can be considered (only for FB15k-237, not for WN18RR).

% For Distmult and TransE, the modifications 
\subsection{DistMult, TransE and ComplEX}
Originally, by its respective authors, both DistMult and TransE models were proposed to be trained using margin loss for ranking. But following the specifications of open source implementation of Distmult in RotatE, we used SoftMargin loss for training as this improves results for the model with both baseline version and with Neighbors' Loss. To implement Neighbors' Loss for these two models we simply augment each minibatch with its neighboring triplets, as defined in equation \ref{eqn:neighbors}, and randomly generated negative samples as per those new triplets. Similar protocol was followed for ComplEX also.

\subsection{RotatE} 
RotatE uses adversarial loss, which is a re-weighted version of the softmargin loss (Equation \ref{eqn:rotate}). We follow the same protocol even when implementing Neighbors' Loss for RotatE. The newly introduced negative samples were also reweighted as per the adversarial loss.

\subsection{TuckER-NL}
As mentioned in previous section TuckER model predicts probability for all target entities given a $(s,o)$ pair, and unlike others is trained with binary cross-entropy loss (see equation \ref{eqn:vanilla-tucker}). Hence, for TuckER it is not always the case that for an entity present in a minibatch there would be only one triplet present. There can be multiple true triplets of the form $(s,r,x)$ for $x \in E$, and all of these will be considered in a minibatch when considering $(s,o)$. But this is still different from Neighbors' Loss as the loss computed for the minibatch would be biased towards a single relation. Hence, to implement Neighbors Loss in TuckER while making the minimal change to the model, for a given subject entity $s$, we first sampled a set of $(s,r')$ pairs and considered them for compuation of the loss in a minibatch.


==> mycontent/optional.tex <==
%% Tucker Theory (REMOVED)

\subsection{TuckER}
\todo{Remove TuckER, not suitable for RWR based sampling!}
The TuckER model \cite{tucker} is based on Tucker decomposition \cite{tucker-dec} of the binary tensor representation of a knowledge graph. This model estimates the probability of a triple (s,r,o) as,
\begin{align}
    p_{(s,r,o)} = p(y_{(s,r,o)}=1) &= \sigma(\phi_{TuckER}(e_s, r, e_o)) \nonumber \\
    \phi_{TuckER}(e_s, r, e_o) &= \mathcal{W} \times_1 \mathbf{e_s} \times_2 \mathbf{w_r} \times_3 \mathbf{e_o}
\end{align}

where, 
$\mathcal{W} \in \mathbb{R}^{d_e \times d_r \times d_e}$  is known as the core tensor, $\times_n$ denotes the tensor product along n-th mode. Also, $y_{(s,r,o)} = 1$ denotes that (s,r,o) is a valid fact triplet. The authors proposed a gradient descent based learning algorithm for training the core tensor and the embeddings for entities and relations in above factorization model. They used the following cross-entropy loss function. 

\begin{align}
    L = -\sum_{(s,r)} \Big( \frac{1}{n_e} \sum_{i=1}^{n_e} \big(&y_{(s,r,i)} \log (p_{(s,r,i)}) \nonumber \\
    &+ (1-y_{(s,r,i)}) \log (1 - p_{(s,r,i)}) \big) \Big) \label{eqn:vanilla-tucker} \\
\end{align}

